Ultra-NeRF: Neural Radiance Fields for Ultrasound Imaging

We present a physics-enhanced implicit neural representation (INR) for ultrasound (US) imaging that learns tissue properties from overlapping US sweeps. Our proposed method leverages a ray-tracing-based neural rendering for novel view US synthesis. Recent publications demonstrated that INR models could encode a representation of a three-dimensional scene from a set of two-dimensional US frames. However, these models fail to consider the view-dependent changes in appearance and geometry intrinsic to US imaging. In our work, we discuss direction-dependent changes in the scene and show that a physics-inspired rendering improves the fidelity of US image synthesis. In particular, we demonstrate experimentally that our proposed method generates geometrically accurate B-mode images for regions with ambiguous representation owing to view-dependent differences of the US images. We conduct our experiments using simulated B-mode US sweeps of the liver and acquired US sweeps of a spine phantom tracked with a robotic arm. The experiments corroborate that our method generates US frames that enable consistent volume compounding from previously unseen views. To the best of our knowledge, the presented work is the first to address view-dependent US image synthesis using INR.

==> MIDL 2023 Ultra-NeRF-2/hacks/many-authors-hack.tex <==
% This hack should not be needed anynore as the issue has been fixed upstream in JMLR v1.26 (2020-01-31)
% https://github.com/MIDL-Conference/MIDLLatexTemplate/issues/8
% https://www.dickimaw-books.com/bugtracker.php?action=view&key=141

%\begin{comment}
\makeatletter
% hack the footer of the title page as it doesn't seem to automatically use the et al. version when spanning acros multiple pages
\renewcommand*{\@titlefoot}{\scriptsize\copyright\space\@jmlryear
    \ifanonsubmission
    \space Author(s) names withheld.\hfill
    \else
    \space \@firstauthor\space \emph{et al}.\hfill
    \@reprint
    \fi
  }
\makeatother
%\end{comment}

% \begin{comment}
\makeatletter
% remove the vbox in @jmlrmaketitle which prevents the text to be split across several pages
\renewcommand{\@jmlrmaketitle}{
  % specify the page style in case it spans over several pages. Not sure why this is needed
  \thispagestyle{jmlrtps}%
  % define a new label for the first page as otherwise it starts from 2 in the header
  \label{jmlrstartnew}%
  % hack the spacing to mimick what happens with a vbox
  \null\vspace{-\parindent}\vspace{-2pt}{
  \hsize\textwidth
  \linewidth\hsize
 \jmlrpretitle
  {%
    \def\titletag##1{##1}%
    \@title
  }%
 \jmlrposttitle
 \jmlrpreauthor \@author \jmlrpostauthor
}
% hack the spacing to mimick what happens with a vbox
\vspace{2pt}
}
\makeatother
%\end{comment}

%\begin{comment}
\makeatletter
% hack the footer to use the new counter
\renewcommand*\@jmlrpages{\pageref{jmlrstartnew}--\pageref{jmlrend}}
\makeatother
%\end{comment}

==> MIDL 2023 Ultra-NeRF-2/sections/conclusion.tex <==
% \section{Conclusion}
% We presented a view-dependent ultrasound synthesis method based on NeRF, which learns patient-specific geometry and the appearance of anatomical structures. 
% We demonstrated that viewing-direction awareness and 3D representation of a scene enable the generation of b-mode images from previously unseen views. 
% Results show the feasibility of this method. Since, to our knowledge,this is the first work directly addressing volumetric rendering for ultrasound in NeRF, it facilitates further extensions and application directions. 
% In future works, the method can be adapted even more to fit ultrasound imaging characteristics. 
% First, an improved method could incorporate prior information about an anatomical structure and anatomy-based regularization. 
% Moreover, the assumption about a static scene does not support many real-world medical scenarios in which anatomical structures are subject to deformations due to external and internal forces. 
% We validated our method on synthetic and phantom data, therefore patient data should be addressed in subsequent works.
% % Although we achieved good results on synthetic and phantom data, we have not evaluated our method on patient data due to the lack of adequate datasets, which should be addressed in subsequent works. 
% We believe, that solving these challenges will enable many novel applications in medical imaging beyond b-mode image synthesis.

==> MIDL 2023 Ultra-NeRF-2/sections/discussion.tex <==
\section{Discussion \& Conclusion}
% In this paper, we presented Ultra-NeRF, a framework to learn the appearance and geometry of a scene from US images. 
In this paper, we present Ultra-NeRF, a volumetric \ac{INR} for \ac{US} imaging from a set of 2D \ac{US} B-mode scans. Unlike prior methods, our approach considers the anisotropic characteristics of \ac{US} and addresses \ac{US} volumetric rendering inline with the physics of \ac{US}.
%We have presented Ultra-NeRF, a NeRF for \ac{US}, that learns a neural volumetric implicit representation of 3D \ac{US} from a set of 2D \ac{US}. In contrast to previous methods we reason about impact of the anisotropic characteristics of \ac{US} on implict representation and address \ac{US} volumetric rendering that adhers to physics of \ac{US}.
The experiments corroborate that Ultra-NeRF incorporates information about the viewing direction into a volumetric \ac{INR}, which allows for the view-dependent synthesis of \ac{US} frames, resulting in high-quality B-mode images.
% The experiments corroborate that Ultra-NeRF integrates knowledge about viewing direction into a neural volumetric implicit representation hence enables the view-dependent synthesis of US frames and produces high quality b-mode images (\figureref{fig:frames_spine}). In~\figureref{fig:r2_compounded_compare} we demonstrated that generated frames facilitate consistent volume compounding from unseen viewpoints. 
% We achieve this task by regressing isotropic physical properties of tissue.
% As presented in~\figureref{fig:maps} the network learns to differentiate between a highly reflective structure, such as a rib, and soft tissue with different levels of attenuation. 
% Our rendering method receives isotropic physical properties and incorporates the rendering direction implicitly which enables the synthesis of view-dependent appearance and geometry.
% As illustrated in~\figureref{fig:r2_compounded_compare} and~\figureref{fig:shadow_output}, we showed that Ultra-NeRF can generate acceptable results that allow us to create consistent compounded volumes from unseen views.
%Our rendering method incorporates view-direction direction implicitly which enables the synthesis of viewpoint-dependent appearance and geometry from isotropic parameters. 
Decomposition of a rendered B-mode in the parameter space shown in~\figureref{fig:maps} further illustrates that Ultra-NeRF identifies tissue characteristics leading to differences in observed intensities. For example, it correctly determines a strongly reflective structure (a rib) by regressing a region with a higher reflectance and therefore produces acoustic shadow. 
We encourage the reader to refer to Appendix~\ref{sec:addional_maps} for additional decomposition of final renderings into rendering parameters and qualitative comparison of regressed parameters for the synthetic dataset. 
\begin{figure}
    \floatconts
    {fig:maps}
    {\caption{Example of rendering parameter decomposition for synthetic (top) and phantom (bottom) test-set data. Intermediate maps illustrate each rendering parameter. In the top row, bone exhibits higher levels of both attenuation and scattering compared to other tissue types (fat, liver, and soft tissue). In the bottom row, the bone only shows high levels of scattering. In both rows, highly reflective tissue interfaces are associated with higher reflectance. Inconsistencies in the bottom regions have no effect due to preceding energy absorption.}}
    %{\caption{\text{Intermediate maps illustrating each element of rendering parameter vector \(\theta\).} The rendering component receives these maps from the MLP and computes final intensity values. Each element corresponds to a tissue's physical property. The attenuation map presents weaker attenuation for brighter regions in the reference image. On the reflectance coefficient map, we observe that the method is aware of a highly reflective structure (a rib). The border probability admits higher values for larger intensities suggesting stronger reflections. Scattering density and scattering amplitude define scattering distribution in the image and are the maps.}
    {\includegraphics[width=0.7\textwidth]{gfx/maps_both.png}}
\end{figure}
We propose a physically sound rendering method, however, further progress towards more realistic B-mode rendering requires addressing ray interactions and the Fresnel Effect. As shown in \figureref{fig:l2_compare_frames}, although the method learns accurate geometry, it does not allow to render complex \ac{US} artifacts, such as reverberations. 
Additionally, to improve rendering results, future work may involve using deep learning techniques to establish a point spread function that reflects the underlying backscattering pattern. Another potential area for future research is regularization; the decomposition into parameter space is under-constrained, thus the outcome highly depends on the initial network configuration. 
%Moreover, to achieve better quantitative results future work may consider deep-learning-based methods to determine a PSF that expresses the underlying backscatterting pattern. Another area for future research is regularization: the decomposition into parameter space is under-constrained, therefore results highly depend on the network initialization. 
To the best of our knowledge, this is the first work that explores the potential of implicit neural representations for medical US by addressing a rendering method specially designed for \ac{US}. Therefore, it supports progress towards integrating the implicit 3D \ac{US} representation exemplified with NeRF into medical applications. 
We believe that this work will inspire further exploration of implicit representations in \ac{US} imaging for medical purpose.
% However, assuming a single ray per a scan-line does not facilitate reproduction of complex \ac{US} artifacts. For instance, reverberations caused by bone tissue produce numerous reflections that appear in a b-mode image (\figureref{fig:frames_spine}). We can therefore observe that Ultra-NeRF's rendering method prioritizes reproduction of strong reflections over artifacts.
% Despite grounding our rendering function in the physics of US, the underlying model approximates physical phenomena related to US wave propagation in tissue. 
% Therefore, the network does not reproduce US artifacts that are not explained by the model.
% For instance, reverberations caused by bone tissue produce numerous reflections that appear in a b-mode image (\figureref{fig:frames_spine}). 
% However, our model assumes that if a high-intensity signal is produced, the remaining energy is lower than the total intensity observed in a b-mode image along one scan-line. 
% The network, therefore, has to decide whether to generate strong reflections or artifacts caused by an echoing sound. 
% In the current network configuration, the network prioritizes creating strong reflections over artifacts.
% Moreover, the rendering procedure samples a scene with a single ray per scan-line, which does not express more complex ray interactions, reflections, or refractions. 
% This is a potential bottleneck for real-world applications of high-quality US synthesis and volume representation. 
% An additional shortcoming of the model is an engineered PSF, which assumes two axes in the image plane and a discrete grid approximation, and does not produce scattering patterns visible in the b-mode images.
% As shown in \figureref{fig:frames_spine}, although the method learns accurate geometry, appearance diverges considerably, which might explain modest quantitative results ($\text{maximum } SSIM_{median} = 0.57$) (Table 1).
% Intermediate maps showing input vectors of the rendering function (\figureref{fig:maps}) illustrate another shortcoming of Ultra-NeRF, namely, large number of independent parameters representing degrees of freedom in output intensity. 
% Large variation in possible outputs leading to the same intensity indicates that the unconstrained network might not provide a unique solution to the same queries between multiple training instances.
% For example, as shown in~\figureref{fig:maps}, if the model's task is to reproduce a low scattering region, the network can compensate a high scattering density by a small amplitude. However, the same result would be produced by a high amplitude and a low scattering density.
% The learnt parameters correlate with physical quantities, however, the values do not reflect actual characteristics of underlying tissue, therefore cannot be interpreted as such. 
% For instance, the unknown TCG factor does not allow us to learn a true distribution of attenuation values, which are compensated and subject to device-specific settings. 
% This could be one of the reasons for the observed discrepancy in attenuation and scattering density (\figureref{fig:maps}) within a tissue that cannot be explained by its heterogeneity. 
% These facts, along with the high degree of freedom and settings-dependence, might result in the same tissue being represented by different intermediate maps. 
% In future works, these shortcomings could be addressed by providing an anatomical prior information, uncertainty measures, and regularization. Like the original NeRF, our model is scene-specific, meaning that it cannot generalize beyond one patient and scanning setup. Furthemore, it is randomly initialized and we expect the model to train only from available images, which results in long training time and unstable training. Anatomical priors, and more complex network architectures might help to address these challenges.

==> MIDL 2023 Ultra-NeRF-2/sections/experiments.tex <==
% \begin{figure}[ht]
% \floatconts
%     {fig:frames_spine}
%     {\caption{Our method infers novel views in phantom and synthetic data (bottom row). However, it does not produce artifacts inconsistent with our ray-based model, such as reverberations (blue), and it fails at representing complex structures (yellow).}}
%     %{\caption{\textbf{B-mode image synthesis.} Our method can infers novel views, as shown in the examples. However, it does not produce artifacts inconsistent with a ray-based model, such as reverberations (blue), and it has failure modes when representing complex structures (yellow).}}
%     {\includegraphics[width=0.9\textwidth]{gfx/frames2.png}
%     }
% \end{figure}
\section{Experiments \& Results}\label{sec:results}
\textbf{Data.} We acquired two types of data: synthetic and phantom B-mode images. For both datasets sweeps were recorded with different, constant perpendicular and tilt angles w.r.t acquisition direction (\figureref{fig:ray}b). We tested our method on 6 sweeps covering views not present in the training set. We encourage the reader to refer to Appendix~\ref{sec:appendix_data} for details about the datasets. \\
%\input{tables/results_ssim}
% \begin{figure}[htbp]
% \floatconts
%     {fig:input_spine}
%     {\caption{\textbf{Spine phantom data.} The first row shows fused sweeps from all views that serve as input to the model. As shown, throughout the training a network receives complete information about the underlying scene. The second row is a compounding from all training data with examples of tilted views illustrated in black in the two last images. The last row illustrates overlaid sweeps and presents how different views contribute to the total volumetric information; red, green, and blue intensities are captured from different view directions.}}
%     {\includegraphics[width=0.5\textwidth]{gfx/input_data.png}}
% \end{figure}
% \textbf{Results.} We evaluated our Ultra-NeRF method both quantitatively and qualitatively.\\
\noindent\textbf{Quantitative Results.} Table~\ref{tab:ssim} presents evaluation of the quality of novel view synthesis as measured in terms of SSIM between synthetic and reference testing data. To analyze the effect of rendering, we compared Ultra-NeRF to an implicit neural representation model without rendering. With rendering, we achieve better or similar results on our phantom data ($\text{SSIM}_{median} = 0.54$ for tilted and $\text{SSIM}_{median} = 0.58$ for perpendicular views), whereas the method without rendering attains higher SSIM values on our synthetic dataset ($\text{SSIM}_{median} = 0.50 \text{ for tilted, } \text{SSIM}_{median} = 0.54 \text{ for perpendicular}$).
%
% \input{tables/results_ssim}
% \begin{figure}[ht]
% \floatconts
%     {fig:shadow_output}
%     {\caption{\textbf{Sagittal plane of compounded volumes.} Volume (a) is the reference compounded from a perpendicular test view of a liver. Volume (b) is compounded from data generated with Ultra-NeRF and volume (c) with the network without rendering. Our method is able to infer view-dependent changes in appearance resulting in the shadow adjusted to the viewing-direction.}}
%     {\includegraphics[width=0.7\textwidth]{gfx/volume_liver_output.png}}
% \end{figure}\\
\input{tables/results_ssim}
\\\noindent\textbf{Qualitative Results.}
To showcase the advantages of our method, we evaluated against explicit 3D representation using volumetric compounding, proposed by~\cite{wachinger2007three}, and a variant of our method without rendering. The results can be seen in \figureref{fig:l2_compare_frames}.
% In \figureref{fig:l2_compare_frames},
%illustrates examples of synthetic B-mode images generated with Ultra-NeRF while \figureref{fig:r2_compounded_compare}
% we demonstrate the significance of rendering. 
We evaluated the quality of novel views by comparing slices from volumetric compounding and generated B-mode scans using Ultra-NeRF with and without the rendering function.
% tilted volume
% We cut through the sagittal plane to illustrate that the rendering improved accuracy of image synthesis. We show that the resulting compounding (b) features occlusions visible in the reference data (a). 
% For the spine dataset we chose three representative views of a compounded tilted volume (\figureref{fig:r2_compounded_compare}). 
% The volumes demonstrate the significance of rendering when a vertebra is visible from a tilted view. 
% \begin{figure}[ht]
% \floatconts
%     {fig:r2_compounded_compare}
%     {\caption{Compounded volumes: without rendering (middle row) the model is not aware of the viewing direction hence occluded parts of the lamina are reconstructed (red). By adding the rendering function we introduce view-direction dependency needed to reconstruct anisotropic phenomena.}}
%     {\includegraphics[width=0.85\textwidth]{gfx/volume_compounding.png}}
% \end{figure}\\
% \noindent\textbf{Baseline Comparison.}
% As our baseline method, we select the method proposed by \cite{wachinger2007three}, which is based on explicit representation. This method is employed in ImFusion~\footnote[2]{ImFusion GmbH, Munich, Germany, software version 2.42} and used in clinical applications. 
For comparison against the explicit method, similar to Ultra-NeRF, we use multiple sweeps. We keep 3 for testing and use the rest of the sweeps for compounding a volume. After compounding, we slice the volume based on the probe pose and orientation recorded in the test sweeps. We compare these results with the ones from Ultra-NeRF to show how explicit methods fail to preserve ultrasound's physics-based properties when generating images from novel views.~\figureref{fig:l2_compare_frames}b highlights this phenomena on our spine phantom. In Appendix~\ref{sec:addional_results}, we show more results from multiple views that emphasizes the importance of physics-based rendering for learning the implicit representation and generating images from novel views.
%Qualitative results are shown in~\figureref{fig:l2_compare_frames}.
\begin{figure}
\floatconts
    {fig:l2_compare_frames}
    {\caption{Evaluating performance through test-set views for our phantom (a) and synthetic (c) dataset. In (b) region marked in red on the phantom example shows an effect of occlusion that methods without rendering fail to recreate. The red arrows in (c) highlight a shadow that is reconstructed with errors when rendering is not employed. Reverberations (blue) and complex structures (yellow) are both challenging for our ray-based model (d).}}
    {\includegraphics[width=0.7\textwidth]{gfx/frames_both.png}}
\end{figure}


==> MIDL 2023 Ultra-NeRF-2/sections/intro.tex <==
\section{Introduction}
3D visualization of an anatomy significantly improves our understanding of the underlying pathology, however, most \ac{US} machines used in practice deliver only a single cross-sectional view of an anatomy at a time. Sonographers, through extensive training and clinical expertise, fuse these 2D scans into a 3D model in their minds. 
% The anatomy of a patient has three dimensions. In 2D US imaging, however, we observe only a single cross sectional view of an anatomy at a time. Therefore, a sonographer has to build a 3D understanding from a set of 2D observations. 
% This demanding task requires extensive training and clinical expertise to allow for mental fusion in 3D.
% Moreover, 
The anisotropic nature of \ac{US} imaging contributes to the increased difficulty of this task. Since an image of a specific region in the patient's body depends on the probe position, a mental 3D model is constantly updated with images that may carry contradicting information for the same region.
% Building a three-dimensional mental model of an organ from a set of 2D \ac{US} frames is a demanding task that requires extensive training and clinical expertise to allow for mental fusion in 3D. 
% The anisotropic nature of \ac{US} imaging contributes to the increased difficulty, since an image of a specific region in the patient's body depends on the probe position.
% Therefore, the mental model is constantly updated based on images that may carry different information for the same region. 
Nevertheless, a trained operator approaches this problem effortlessly owing to the consciousness of the anatomy and the effect of the probe position on its 2D representation.
However, this manual visual analysis remains expensive and error-prone~\cite{lyshchik2004three,kojcev2017reproducibility,kronke2022tracked}.
A system that can represent the 3D underlying geometry of an anatomy based on multiple \ac{US} scans can reduce the error rate.

Much research has recently been devoted to utilizing 3D \ac{US} as an explicit way of modeling the geometry. 3D \ac{US} is used in diagnostic applications, as well as interventional radiology. 3D US volumes are conventionally generated using special wobbler probes, 2D transducers, or tracked probes to compound a 3D volume from 2D slices~\cite{busam2018markerless}. In the last decade, new approaches such as computational sonography~\cite{hennersperger2015computational}, sensorless 3D US~\cite{prevost2017deep}, and deep learning-based image formation techniques~\cite{Simson18} have aimed at improving the 3D compounding quality of this portable and affordable modality. %The anisotropic nature of the US modality generates various view-dependent artifacts which have negative effects on multi-modal medical imaging applications.
However, none of these approaches can properly model the underlying scene. When looked at the compounded volume from different views, the resulting B-mode image is not a plausible one. As an example, when slicing from a novel view, acoustic shadows might be displayed where there is should be none or an anatomy shown where no rays could possibly reach it from this novel view. However, with a correct modeling, one can generate plausible B-mode scans from any arbitrary view.
Our proposed approach focuses on learning the underlying geometry using 2D US images from different viewpoints.
% This method enables us to generate isotropic 3D US volumes, which introduces a new intermediate modality for the medical image processing community to explore. 
Our method enables us to generate physically plausible B-mode scans from novel views and introduces a new implicit US representation for the medical image processing community to explore.

Although viewing-direction dependency is a prominent characteristic of US imaging, it is not a unique property of US.
To some extent, a similar phenomenon characterizes natural images. For instance, since the non-Lambertian assumption does not hold for most real world objects, appearance due to reflections might be inconsistent between views~\cite{gao2022polarimetric}. 
3D scene reconstruction from a set of 2D view-dependent observations has been hence extensively studied~\cite{seitz1999photorealistic,niemeyer2020differentiable}. An important aspect of any reconstruction method is a scene representation, which can be either explicit (e.g. volumetric grids), or implicit (e.g. implicit functions).
Implicit scene representations, such as (truncated) signed distance functions ((T)SDFs)~\cite{newcombe2011kinectfusion} represent a 3D scene as a function. Since neural networks are universal function approximators, they can be used to parametrize an implicit representation~\cite{tewari2022advances}. This fact has been a basis of a recent development in neural volumetric representation. In particular, \ac{NeRF} emerged as a new, potent method for generating photorealistic, view-dependent images of a static 3D scene from a collection of pose-annotated images~\cite{NeRF2022}. 
In computer vision,
% NeRF became a baseline for a prolific research addressing various aspects such as dynamic scenes~\cite{park2021nerfies}, large scale scenes~\cite{rematas2022urban}, or scene generalization~\cite{yu2021pixelnerf}.
\ac{NeRF} became a baseline for  for various research directions such as dynamic scenes~\cite{park2021nerfies}, large scale scenes~\cite{rematas2022urban}, or scene generalization~\cite{yu2021pixelnerf}.
Moreover, as presented in iNeRF~\cite{yen2021inerf} representing a 3D model as a neural network provides a reference for 6DoF pose estimation, which potentially can find an application in US tracking.
The idea behind \ac{NeRF}, however, was primarily developed for natural image synthesis and takes advantage of established methods from computer graphics. 

% In particular, it builds on a ray-based rendering formulation~\cite{kajiya1984ray} whose underlying physics is unsuitable to an US image formation model.\\
In this paper, for the first time, we propose an implicit neural representation with physics-based rendering for \ac{US} imaging exemplified with NeRF that facilitates the synthesis of B-mode images from novel viewpoints. 
Our contributions are as follows: 
\begin{itemize}
\setlength\itemsep{0em}
    \item a method that synthesises accurate B-mode images by learning the view-dependent appearance and geometry of a scene from multiple US sweeps;
    \item a physically sound rendering formulation based on a ray-tracing model, which considers the isotropic tissue characteristics important to \ac{US};
    \item open source datasets\footnote{The link to the data and implementation will be provided upon acceptance.} comprising multiple tracked 2D \ac{US} sweeps with highly accurate pose annotations and different viewpoints.
\end{itemize}
In our experiments, we use synthetic liver and spine phantom data.
We evaluate our method quantitatively and qualitatively.
In particular, we demonstrate the importance of rendering based on the physics behind US imaging and the shortcomings of learning an INR without considering view-dependent changes to the observed scene.
To the best of our knowledge, this paper presents a new implicit neural representation for \ac{US} that for the first time considers the anisotropic characteristics of US. 
% first application of NeRF to ultrasound that considers view-dependent characteristics of ultrasound imaging.

==> MIDL 2023 Ultra-NeRF-2/sections/method.tex <==
\section{Method}
\begin{figure}
\floatconts
    {fig:model}
    {\caption{
     \textbf{a)} For a query point $ q \in \mathbb{R}^{3}$ sampled along a ray, the MLP estimates a parameter vector $\theta \in \mathbb{R}^{5}$ from an implicit volume representation, \textbf{b)} from parameters at queried and preceding positions along the ray the rendering computes a per-query intensity. Resulting intensities compose an \ac{US} image. The output and target frame are compared using a weighted sum of Structural Similarity Index Measure (SSIM) and Squared Error Loss (L2).
    }
    }
    %\textbf{Proposed framework in the single-frame case.} The method consists of two modules: (a) a multi-layer perceptron (MLP) and (b) volume rendering function. 
    %For a query point $\textbf{q} \in \mathbb{R}^{3}$ sampled along a probe ray, the network extracts a parameter vector $\theta \in \mathbb{R}^{5}$ from an internal volume representation. Once all the queries along the ray are computed, the resulting vectors are passed to the rendering function.
    %The rendering computes a per-query intensity that depends on parameters at queried and preceding positions along the ray. To render the complete image, we query rays covering a complete image space. Finally, we composite the pixel intensities into an image. The output frame is compared with the target image using SSIM.}
    {\includegraphics[width=\textwidth]{gfx/network3.png}}
\end{figure}
\subsection{Background: US Physics}
US images are generated by mapping reflected sounds from the tissue within a thin transversal slice of the body. As an anisotropic modality, US exhibits varying behavior in different types of tissue, resulting in direction-dependent differences in the resulting echoes. This characteristic underscores the importance of accounting for tissue anisotropy in the methods generating B-mode images.
Intrinsic acoustic parameters such as travelling speed of sound, acoustic impedance, attenuation coefficient, and spatial distribution of sound scattering micro-structures are the main contributing factors affecting the sound reflection within the tissue. 
By knowing the mapping of these parameters in space and the wave propagation direction, one can simulate renderings of 3D US in arbitrary views~\cite{salehi2015patient}. 
% \begin{figure}[htbp]
%  % Caption and label go in the first argument and the figure contents
%  % go in the second argument
% \floatconts
%   {fig:example}
%   {\caption{Example Image}}
%   {\includegraphics[width=0.5\linewidth]{example-image}}
% \end{figure}
% \begin{figure}[ht]
% \floatconts
%     {fig:ray}
%     {\caption{a) Each ray \begin{math} r(t) \end{math} corresponds to a single scan-line oriented perpendicularly to the acquisition direction \begin{math} d \end{math} and with origin \begin{math} o \end{math} at top of the image plane. Query points are defined by their spatial location in a 3D volume (\begin{math} r(t) = o + td \end{math}).b) White intensities are the result of max-value compounding of images from all available angles. Red/Blue/Green intensities show the composition of the white intensities based on their view angle. }
%     %{\caption{\textbf{A ray and query points.} Each ray \begin{math} r(t) \end{math} corresponds to a single scan-line with origin \begin{math} o \end{math} at top of the image plane and traverses through the medium perpendicularly to the
%     %acquisition direction \begin{math} d \end{math}. Along each ray we sample a set of query points defined by \begin{math} r(t) = o + td \end{math} that correspond to the spatial location within a 3D volume.}
%     }
%     {\includegraphics[width=0.9\textwidth]{gfx/data.png}}
% \end{figure}
\subsection{Ultrasound NeRF}
\figureref{fig:model} presents our framework in the single-frame case. The method follows the original NeRF w.r.t its two components: a neural network (\figureref{fig:model}a) and volumetric rendering (\figureref{fig:model}b). 
The network represents a volume as a 3D vector-valued continuous function that maps a position $q = (x, y, z) $ in a Cartesian coordinate space into a parameter vector $\theta \in \mathbb{R}^{5}$ which elements correspond to attenuation $\alpha$, reflectance $\beta$, border probability $\rho_{b} $, scattering density $\rho_s$, and scattering intensity $\phi$ and compose a final pixel intensity as outlined in Section~\ref{sec:rendering}. The parameter vector consists of isotropic physical tissue properties hence we do not provide explicit viewing directions to the network.
% These parameters serve as input to the rendering function. 
%because the parameter vector consists of isotropic physical tissue properties.
This ensures that the regressed physical properties remain consistent between views, whereas the view-dependent changes are enforced by the rendering.
%which implicitly receives viewing directions from a set of queries along a ray.
Figure~\ref{fig:ray} illustrates definition of a ray and query points. We encourage the reader to refer to Appendix~\ref{sec:network} for the network details.
%%%%%%%%%%%%
\subsection{Ultrasound Volume Rendering} \label{sec:rendering}
Our US volume rendering model builds upon a formulation presented by~\citet{salehi2015patient} that proposes a ray-tracing-based simulation model. The advantage of this model is its flexibility in representing US artifacts coming from backscattering effects.

For each scan-line \(r\), Equation~\ref{eq:total_echo} defines a recorded US echo \(E(r, t)\), measured at distance \(t\) from the transducer, as a sum of reflected \(R(r, t)\) and backscattered \(B(r, t)\) energy:
\begin{equation} \label{eq:total_echo}
    E(r, t) = R(r, t) + B(r, t)
\end{equation}
The reflected energy is defined by:
\begin{equation} \label{eq:reflected_energy}
    R(r, t) = | I(r, t) \cdot \beta(r, t)| \cdot PSF(r) \otimes G(r', t')
\end{equation}
Where $\otimes$ is the convolution operator, \(I(r,t)\) is the remaining energy at the distance \(t\), \(\beta(r, t)\) represents the reflection coefficient, and \(PSF(r)\) is a predefined 2D point-spread function. G(r, t) admits 1 for points at the boundary and 0 otherwise. We compute it by sampling from a Bernoulli distribution parameterized by the border probability $\rho_b$. A probabilistic approach to the border definition reflects network's uncertainty about interaction of the ray with a tissue border.
% We use a probabilistic approach because the underlying anatomical structure is unknown therefore we do not know the position of the tissue borders. 
The energy loss is traced along each scan-line, and the remaining energy \(I(r, t)\) is modelled using the loss of the energy due to reflection \(\beta\) at the boundaries and attenuation compensated by applying an unknown time-gain compensation (TGC) function. The final formulation for \(I(r, t)\) assumes an initial unit intensity \(I_0(r, 0)\) and loss of energy at each step \(dt\).
% \begin{equation} \label{eq:remaining_intensity_full}
% I(r, t) = I_0 \cdot \prod_{n=0}^{t-1}{[(1 - \beta(r, n)) \cdot G(r, n)]} \cdot \exp^{(-\int_{n=0}^{t-1}{(\alpha - TGC_n) \cdot f \cdot dt)}}
% \end{equation}
We can further simplify the resulting equation by modeling the compensated attenuation \(\alpha\) by a single parameter since TGC is a scaling factor:
\begin{equation} \label{eg:remaining_intensity_short}
I(r, t) = I_0 \cdot \prod_{n=0}^{t-1}{[(1 - \beta(r, n)) \cdot G(r, n)]} \cdot \exp^{(-\int_{n=0}^{t-1}{(\alpha \cdot f \cdot dt))}}
\end{equation}
Consequently,
\(\alpha's\) correspond to the physical attenuation only up to an unknown scaling factor.
The backscattered energy \(B(r, t)\) from the scattering medium is a function of remaining energy \(I(r, t)\) and a 2D map of scattering points \(T(r, t)\):
\begin{equation} \label{eq:backscattering}
B(r, t) = I(r, t) \cdot PSF(r) \otimes T(r', t')     
\end{equation}
The map \(T(r, t)\) is learnt using a generative model inspired by~\cite{zhang2020deep}:
\begin{equation} \label{eq:scattering_template}
    T(r, t) = H(r, t) \cdot \phi(r, t)
\end{equation}
In this model, \(H(r,t)\) admits 1 for a query point being a scattering point and 0 otherwise. This function is sampled from the Bernoulli distribution parameterized by scattering density \(\rho_s\). It represents the uncertainty of whether the scattering effect of a scattering point is observed. The intensity of a scattering point is controlled by its amplitude \(\phi\) which models sampling from a normal distribution with the mean \(\phi\) and unit variance.
We address differentiability of the model in Appendix~\ref{sec:differentiability}.
% ~\subsection{Network Structure}
% Our network is a fully-connected network, known as a multi-layer perceptron (MLP). It consists of 8 layers with 128 neurons. As discussed in~\cite{NeRF2022}, we are using positional encoding on an input vector, which maps it to a higher dimensional space to help the network learn high-frequency details. We are optimizing the weights of our network using the Adam optimizer~\cite{kingma2014adam}. Our loss is a weighted sum of Structural Similarity Index Measure (SSIM)~\cite{wang2004image} and Squared Error Loss (L2) between the rendered and true b-mode images.
\begin{figure}
\floatconts
    {fig:ray}
    {\caption{(a) Each ray \begin{math} r \end{math} corresponds to a single scan-line with origin \begin{math} \textbf{o} \end{math} at top of the image plane and direction \begin{math}\textbf{d} \end{math} pointing along the scan-line. Query points are defined by their spatial location \begin{math} \textbf{r}(t) = \textbf{o} + t\textbf{d} \end{math}. (b) Visualization of the phantom dataset: white intensities (top) from max-value compounding of all-angle images; red/blue/green intensities (bottom) compose white intensities by view angle; middle row visualizes observation directions with respect to anatomy.}
    
    % This visualization depicts input from the phantom dataset: white intensities (top) result from max-value compounding of images from all angles; red/blue/green intensities (bottom) compose white intensities by view angle; middle row visualizes observation directions w.r.t anatomical structure}
    %{\caption{\textbf{A ray and query points.} Each ray \begin{math} r(t) \end{math} corresponds to a single scan-line with origin \begin{math} o \end{math} at top of the image plane and traverses through the medium perpendicularly to the
    %acquisition direction \begin{math} d \end{math}. Along each ray we sample a set of query points defined by \begin{math} r(t) = o + td \end{math} that correspond to the spatial location within a 3D volume.}
    }
    {\includegraphics[width=0.8\textwidth]{gfx/data.png}}
\end{figure}

==> MIDL 2023 Ultra-NeRF-2/sections/related_work.tex <==
\section{Related Work}
% \textbf{Implicit representation.} 
Implicit representations in the form of (T)SDFs have been used for implicit geometric reconstruction~\cite{newcombe2011kinectfusion}. 
% Recently, {\it implicit representation}~\cite{sitzmann2020implicit}, a novel method of representing signals as a neural network proved to be a convenient way for storing information about a 3D scene. 
% Recently, it proved to be a convenient way for storing information about a 3D scene by representing signals as a neural network~\cite{sitzmann2020implicit}. 
Recently, INR has been proposed to express signals as a neural network~\cite{sitzmann2020implicit} which can be seen as a universal function approximator, which represents a scene as a continuous function parameterised by its weights.
As a consequence, it allows for a mapping from a 3D continuous coordinate space to intensity to store information about a 3D scene.As presented by~\citet{gu2022representing}, we can exploit INR models to represent a 3D US volume learnt from a set of 2D US images. However, parametrizing an US volume using a 3D continuous coordinate space does not address a viewing direction impact on the observation.
% As discussed in ImplicitVol~\cite{yeung2021implicitvol}, implicit volume representation enables the extraction of any cross-sectional plane; therefore can be used as a training signal for sensorless volume reconstruction. 
% In IREM, the authors propose an image reconstruction framework based on implicit representation, which reproduces high-resolution magnetic resonance (MR) images using low-resolution training data~\cite{wu2021irem}. 
% In US imaging an INR stores a volume learnt from a set of US frames~\cite{gu2022representing}. 
% However, the observed geometry and appearance of a specific location might be inconsistent when the location is present in more than one image, since US is a view-dependent modality. 
% Therefore, an implicit representation in US might be inadequate to represent view-dependent changes in the scene's geometry and appearance.\\
% \textbf{Neural Radiance Field.} 
The progress in neural continuous shape representation sparked interest in their application to photorealistic novel view synthesis.
In particular, in a seminal work introducing \ac{NeRF}~\cite{NeRF2022}, the authors propose a framework that combines neural representation of a scene and fully differentiable volumetric rendering.
In \ac{NeRF}, the representation of a scene is expressed by a fully-connected neural network. The network maps a 5D vector (a spatial location 
$\textbf{x}$ and viewing direction
$\textbf{d}$) to volume density
$\sigma$,
and radiance 
$\textbf{c}$. 
To learn this mapping a per-pixel camera ray is defined as $\textbf{r}(t) = \textbf{o} + t\textbf{d}$
with the camera origin $\textbf{o}$
in the center of the pixel defining the near plane.
% The final colour value of each pixel is calculated using a rendering method that considers contribution of density and radiance at each spatial location along a ray as defined by following formulas:
The final colour value of each pixel is defined by following formulas:
\begin{equation} \label{eq:nerf1}
    C(\textbf{r}) = \int_{t_n}^{t_f} T(t)\sigma(t)c(t)dt
\end{equation}
\begin{equation} \label{eq:nerf2}
\text{where } 
    T(t) = \exp{-\int_{t_n}^{t_f}}\sigma(\textbf{r}(s))ds
\end{equation}
The volume rendering integral in~\equationref{eq:nerf1} accumulates ray-traced radiance field from near $t_n$ to far plane $t_f$, with each position contributing to the final pixel color. 
The input of each sample is controlled by the transmittance factor \(T(t)\) (\equationref{eq:nerf2}).
% The transmittance can be further interpreted as a probability that the ray does not terminate between $t_n$ and $t_i$. 
Finally, the rendered pixel value is compared with a value in an image using a photometric loss.

Since its introduction, \ac{NeRF}-based methods have demonstrated impressive results in various fields including medical imaging.
% Due to its flexibility and high quality of novel view synthesis NeRF has been been recently applied in medical imaging. 
For instance, MedNeRF propose a \ac{NeRF} framework to reconstruct CT-projections from X-ray~\cite{corona2022mednerf}, and EndoNeRF adopts \ac{NeRF} for surgical scene 3D reconstruction~\cite{wang2022neural}.
% Yet, researchers have not thoroughly investigated the potential of NeRF in the context of US imaging. 
Yet, surprisingly little investigation has been done to explore the potential of neural volumetric implicit representations for medical US.
One of a few studies~\cite{yeung2021implicitvol, gu2022representing, song2022development} focuses on reconstruction of a spine using the \ac{NeRF} algorithm~\cite{li20213dspinenerf}. 
In this paper, the authors demonstrate that \ac{NeRF} can render high-quality US images.
However, they apply \ac{NeRF} without considering a volumetric rendering method, which respects US physics. % the accumulation of information along the ray (\equationref{eq:nerf1}) does not respect the physics of the US acquisition process.
%is not justified by the US image formation.
To address this shortcoming, we reformulate the rendering step to include the underlying US physics and incorporate it into the \ac{NeRF} framework.
%instead focus on reformulating rendering such that it is based on the physics of US.
% \begin{figure}[ht]
% \floatconts
%     {fig:model}
%     {\caption{
%     Proposed framework in the single-frame case: a) For a query point $\textbf{q} \in \mathbb{R}^{3}$ sampled along a probe ray, the MLP extracts a parameter vector $\theta \in \mathbb{R}^{5}$ from an internal volume representation, b) the rendering computes a per-query intensity depending on parameters at queried and preceding positions along the ray. Then we compose the pixel intensities into an image. %The output and target frame are compared using %SSIM.
%     }
%     }
%     %\textbf{Proposed framework in the single-frame case.} The method consists of two modules: (a) a multi-layer perceptron (MLP) and (b) volume rendering function. 
%     %For a query point $\textbf{q} \in \mathbb{R}^{3}$ sampled along a probe ray, the network extracts a parameter vector $\theta \in \mathbb{R}^{5}$ from an internal volume representation. Once all the queries along the ray are computed, the resulting vectors are passed to the rendering function.
%     %The rendering computes a per-query intensity that depends on parameters at queried and preceding positions along the ray. To render the complete image, we query rays covering a complete image space. Finally, we composite the pixel intensities into an image. The output frame is compared with the target image using SSIM.}
%     {\includegraphics[width=\textwidth]{gfx/network4.png}}
% \end{figure}

==> MIDL 2023 Ultra-NeRF-2/tables/dataset_table.tex <==
\begin{table}[ht]
    \footnotesize
    \centering
    \setlength{\tabcolsep}{2 pt}
    \floatconts
    {tab:dataset}%
    {\caption{Dataset test-train split.}}%
    {\begin{tabular}{cc cccc cccc}
        \toprule
    \multicolumn{2}{c}{}&  \multicolumn{2}{c}{synthetic} & \multicolumn{2}{c}{phantom}   \\
        % \cmidrule(lr){3-6} \cmidrule(lr){7-10}
    % \multicolumn{2}{c}{}  &  liver synthetic & & spine phantom\\
    \toprule
        % \multicolumn{2}{c}{}&  \multicolumn{2}{cc}{training & testing} & \multicolumn{4}{2}{training & testing}   \\
    \multicolumn{2}{c}{dataset type}  & training & testing & training & testing\\
        \midrule
            & number of sweeps     & 4 & 3      & 8 & 3\\
            & number of frames & 800 & 600 & 1200 & 300\\
        \addlinespace
        \bottomrule
    \end{tabular}}
\end{table}

% \begin{table}[ht]
%     \footnotesize
%     \centering
%     \setlength{\tabcolsep}{2 pt}
%     \floatconts
%     {tab:dataset}%
%     {\caption{Dataset splits}}%
%     {\begin{tabular}{cc cccc cccc}
%         \toprule
%     \multicolumn{2}{c}{}&  \multicolumn{4}{c}{liver synthetic} & \multicolumn{4}{c}{spine phantom}   \\
%     \multicolumn{2}{c}{}&  \multicolumn{4}{c}{training & testing} & \multicolumn{4}{c}{training & testing}   \\
%         % \cmidrule(lr){3-6} \cmidrule(lr){7-10}
%     % \multicolumn{2}{c}{}  & liver synthetic & & spine phantom\\
%     \toprule
%     % \multicolumn{2}{c}{dataset type}  & training & testing & training & testing\\
%     % \cmidrule(lr){3-6} \cmidrule(lr){7-10}
%         \midrule
%             & number of sweeps     & 4 & 3      & 8 & 3\\
%             & number of frames & 800 & 600 & 1200 & 300\\
%         \addlinespace
%         \bottomrule
%     \end{tabular}}
% \end{table}

==> MIDL 2023 Ultra-NeRF-2/tables/results_ssim.tex <==
\begin{table}
    \footnotesize
    \centering
    \setlength{\tabcolsep}{2 pt}
    \floatconts
    {tab:ssim}%
    {\caption{SSIM between synthetic and reference B-mode images.}}%
    {\begin{tabular}{cc cccc cccc}
        \toprule
    \multicolumn{2}{c}{}&  \multicolumn{4}{c}{with rendering} & \multicolumn{4}{c}{w/o rendering}   \\
        \cmidrule(lr){3-6} \cmidrule(lr){7-10}
    \multicolumn{2}{c}{dataset type}  & median  & mean  &  min  & max  & median  & mean  &  min  & max\\
        \midrule
    \multirow{2}{*}{liver synthetic} 
            & tilted     &   0.47  & 0.45    &  0.41   & 0.60    & \textbf{0.50} & 0.51 & 0.46 & 0.59\\
            & perpendicular & 0.49    & 0.49   & 0.44    & 0.57   & \textbf{0.54}   & 0.54 & 0.47 & 0.62\\
        \addlinespace
    \multirow{2}{*}{spine phantom} 
            & tilted & \textbf{0.54} & 0.51 & 0.36 & 0.60 & 0.50 & 0.48 & 0.36 & 0.59\\
            & perpendicular & \textbf{0.58} & 0.54    & 0.42   & 0.65    & \textbf{0.58}    & 0.54 & 0.41 & 0.64\\
        \addlinespace
        \bottomrule
    \end{tabular}}
\end{table}

==> hacks/many-authors-hack.tex <==
% This hack should not be needed anynore as the issue has been fixed upstream in JMLR v1.26 (2020-01-31)
% https://github.com/MIDL-Conference/MIDLLatexTemplate/issues/8
% https://www.dickimaw-books.com/bugtracker.php?action=view&key=141

%\begin{comment}
\makeatletter
% hack the footer of the title page as it doesn't seem to automatically use the et al. version when spanning acros multiple pages
\renewcommand*{\@titlefoot}{\scriptsize\copyright\space\@jmlryear
    \ifanonsubmission
    \space Author(s) names withheld.\hfill
    \else
    \space \@firstauthor\space \emph{et al}.\hfill
    \@reprint
    \fi
  }
\makeatother
%\end{comment}

% \begin{comment}
\makeatletter
% remove the vbox in @jmlrmaketitle which prevents the text to be split across several pages
\renewcommand{\@jmlrmaketitle}{
  % specify the page style in case it spans over several pages. Not sure why this is needed
  \thispagestyle{jmlrtps}%
  % define a new label for the first page as otherwise it starts from 2 in the header
  \label{jmlrstartnew}%
  % hack the spacing to mimick what happens with a vbox
  \null\vspace{-\parindent}\vspace{-2pt}{
  \hsize\textwidth
  \linewidth\hsize
 \jmlrpretitle
  {%
    \def\titletag##1{##1}%
    \@title
  }%
 \jmlrposttitle
 \jmlrpreauthor \@author \jmlrpostauthor
}
% hack the spacing to mimick what happens with a vbox
\vspace{2pt}
}
\makeatother
%\end{comment}

%\begin{comment}
\makeatletter
% hack the footer to use the new counter
\renewcommand*\@jmlrpages{\pageref{jmlrstartnew}--\pageref{jmlrend}}
\makeatother
%\end{comment}
